Amplifiers of selection for the Moran process with both Birth-death and death-Birth updating

Populations evolve by accumulating advantageous mutations. Every population has some spatial structure that can be modeled by an underlying network. The network then influences the probability that new advantageous mutations fixate. Amplifiers of selection are networks that increase the fixation probability of advantageous mutants, as compared to the unstructured fully-connected network. Whether or not a network is an amplifier depends on the choice of the random process that governs the evolutionary dynamics. Two popular choices are Moran process with Birth-death updating and Moran process with death-Birth updating. %Moran process has two popular versions called Birth-death updating and death-Birth updating. Interestingly, while some networks are amplifiers under Birth-death updating and other networks are amplifiers under death-Birth updating, no network is known to function as an amplifier under both types of updating simultaneously. In this work, we identify networks that act as amplifiers of selection under both versions of the Moran process. The amplifiers are robust, modular, and increase fixation probability for any mutant fitness advantage in a range $r\in(1,1.2)$. To complement this positive result, we also prove that for certain quantities closely related to fixation probability, it is impossible to improve them simultaneously for both versions of the Moran process. Together, our results highlight how the two versions of the Moran process differ and what they have in common.

==> positive-explicit.tex <==
\section{Explicit result for fixed $n$ and $r\to 1$}

In this section we prove~\cref{thm:positive-r1}.
%The above construction works for all large enough population sizes.
%here we analyze a related specific construction for fixed $n$ and in the limit $r\to 1$.

%\subsection{Construction}
\newcommand{\amp}{A}
\newcommand{\metafan}{metafan}
%\def{\wacross}{w}
\newcommand{\phub}{p_{\operatorname{hub}}}
\newcommand{\slope}{s}

%\pepa{blabla: hub, blades, unit, all-mutant, fire-in, fire-out. Cite NatComm, cite Allen}

First, we describe a family of edge-weighted graphs $\amp_N$ that substantially amplify selection under the Birth-death updating when $r\to 1$.
The graphs $\amp_N$ consist of a large complete graph in the center and several pairs of nodes arranged around it and connected to the central hub via low-weight edges.

Formally, given positive integers $N$ and $b<N/2$, a \textit{\metafan{} on $N$ nodes with $b$ blades}, denoted $\amp_N(b)$, is an edge-weighted graph that consists of a complete graph on $a=N-2b$ nodes (called a \textit{hub}), together with $N/4$ pairs of nodes (called \textit{blades}) arranged around the hub and connected to the hub but not to each other.
When $N$ is divisible by 4, for brevity we denote $\amp_N=\amp_N(N/4)$ the \metafan{} with $N/4$ blades (that is, half the nodes are in the hub and half are in the blades).

To describe the edge weights, we consider a real number $\eps>0$.
The edges within the hub have weight 1,
the edges within the blades have weight $\eps$, and
the edges connecting the blades to the hub have weight $\eps^2$.
When $\eps\to 0$, the edge weights guarantee that the evolutionary dynamics occurs on three different time scales.

First, any time an individual is selected for reproduction, with probability close to 1 the offspring will migrate to another node in the same unit (a hub or a blade).
Thus, in between any two hub-blade interactions, the hub and each blade (individually) resolve to a homogeneous state.
That is, within each unit either all nodes are mutants or all nodes are residents.

Second, occasionally a node in a blade reproduces and the offspring migrates to the hub.
We call this a \textit{fire-in} event.
When $\eps$ is small, a reproduction event is a fire-in event with probability roughly $\eps^2/\eps=\eps\ll 1$. 
If that fire-in event is due to a mutant placing their offspring in the hub, the hub might become all mutants with a certain probability. % $\phubmut$.
Likewise, a resident fire-in might convert the hub to become all residents. % with certain probability $\phubres$.
Since hub evolves on a fast time-scale, it will become homogeneous in between any two fire-in events.
Thus, in the long-term, the hub will spend a certain proportion $\phub\in(0,1)$ of time in the ``all-mutants'' state and the remaining proportion $1-\phub$ of time in the ``all-residents'' state.
Below we will express the quantity $\phub=\phub(k)$ in terms of the number $k$ of blades that are currently all-mutant.

Third, rarely a node in the hub reproduces and the offspring migrates to some blade.
We call this a \textit{fire-out} event.
When $\eps$ is small, a reproduction event is a fire-out event with probability roughly $\eps^2\ll \eps$, thus fire-out events are even much rarer than fire-in events.
As before, a fire-out event might change a blade from all-residents to all-mutants or vice versa.

All in all, the above arguments imply that as $\eps\to 0$, the evolutionary dynamics can be faithfully represented as follows:
%by tracking only the number of all-mutant blades.
%In particular, the fixation probability $\fp(\amp_N,r)$ is given by
% \[
% \fp(\amp_N,r)=\pinblade \cdot \pbladewin \cdot 
% \]
\begin{enumerate}
    \item First, a mutant appears.
    \begin{itemize}
        \item If the mutant appears in the hub, the hub becomes either all mutants or all residents. Either way, due to occasional fire-ins from the blades the hub eventually becomes all residents and the mutants go extinct.
        \item If the mutant appears in a blade then the blade becomes either all mutants (with probability $\frac{r}{r+1}$), or all residents (with probability $\frac1{r+1}$). %In the latter case, mutation went extinct, so assume the former case.
    \end{itemize}
    \item From this point on, it suffices to track only the number $k\in[1,b-1]$ of all-mutant blades. For any number $k$ of all-mutant blades, we compute the probability $p^+(k)$ (resp.\ $p^-(k)$) that a fire-out event leads to one more blade becoming all-mutant (resp.\ all-resident). This computation takes into account the long-term proportion $\phub(k)$ of time that the hub spends being all-mutants, as well as the number $k$ of all-mutant leaves.
    \item Eventually, this 1-dimensional random walk on states $k\in\{0,1,2,\dots,b\}$ with forward bias $p^+(k)/p^-(k)$ results in either 0 all-mutant leaves (this corresponds to mutant extinction), or to $b$ all-mutant blades (this corresponds to mutant fixation).
\end{enumerate}

In what follows we bound the overall fixation probability $\fp(\amp_N,r)$ for any $r\ge 1$ from below. Then, we plug in $r=1+\delta$ for $\delta\to 0$ to find the derivative of $\fp(\amp_N,r)$ with respect to $r$ at $r=1$.

First, we express $\phub(k)$.
Fix $k\in[1,b-1]$ and let $F=k\cdot 2r + (b-k)\cdot 2$ be the total fitness of the sub-population in the blades.
Any fixed reproduction event is a mutant fire-in event with probability proportional to $\frac{2r\cdot k}{F}$, and it succeeds in turning the hub to all-mutants with probability $\fp(K_a)$ for a total rate of $p_m(k)=\frac{2r\cdot k}{F}\cdot\fp(K_a)$.
Similarly, any fixed reproduction event is a resident fire-in event with probability proportional to $\frac{2\cdot (b-k)}{F}$, and it succeeds in turning the hub to all-residents with probability $\rho_{1/r}(K_a)$, for a total rate of $p_r(k)= \frac{2\cdot (b-k)}{F}\cdot \rho_{1/r}(K_a)$.
Thus, the proportion of time $\phub(k)$ that the hub spends in the all-mutant state is
\[
\phub(k) = \frac{p_m(k)}{p_m(k)+p_r(k)} = \frac{rk\cdot \fp(K_a)}{rk\cdot \fp(K_a) + (b-k)\cdot \rho_{1/r}(K_a)}.
\]
Now we turn to computing the ratio $p^+(k)/p^-(k)$. The number of all-mutant blades can change only when a fire-out event occurs. In order to gain an all-mutant blade, the hub must be all-mutant, a hub-node must be selected for reproduction, the offspring must migrate to an all-resident blade, and it must turn it into an all-mutant blade. Thus, the probability $p^+(k)$ is proportional to the product of four terms
\[ \phub(k)\cdot \frac{r\cdot a}{r\cdot (a+2k)+1\cdot 2(b-k)} \cdot \frac{b-k}{b}\cdot\frac{r}{r+1}.
\]
Similarly, the probability $p^-(k)$ is proportional to a product
\[ (1-\phub(k))\cdot \frac{1\cdot a}{r\cdot 2k+1\cdot (a+2(b-k))} \cdot \frac{k}{b}\cdot\frac{1}{r+1}.
\]
The ratio $p^+(k)/p^-(k)$ therefore satisfies
\begin{align*}
\frac{p^+(k)}{p^-(k)}
&= \frac{p_m(k)}{p_r(k)} \cdot \frac{r^2\cdot 2k+r\cdot (a+2(b-k))}{r\cdot (a+2k)+1\cdot 2(b-k)}\cdot \frac{b-k}{k}\cdot r\\
&=r^2\cdot \frac{\fp(K_a)}{\rho_{1/r}(K_a)}\cdot \frac{r^2\cdot 2k+r\cdot (a+2(b-k))}{r\cdot (a+2k)+1\cdot 2(b-k)}\\
&\ge r^2\cdot\frac{\fp(K_a)}{\rho_{1/r}(K_a)}\\
&=r^2\cdot \frac{\frac{1-1/r}{1-1/r^a}}{\frac{r-1}{r^a-1}} = r^{a+1}.
\end{align*}
Using the standard formula for the absorption probability of a random walk with constant forward bias thus yields
\[
\fp(\amp_N,r)\ge \frac{2b}{N}\cdot \frac{r}{r+1}\cdot \frac{1-1/r^{a+1}}{1-1/\left(r^{a+1}\right)^b}.
\]
Specifically, for $r=1+\delta$ we get
\begin{align*}
\fp(\amp_N,1+\delta)
&\ge \frac12\cdot
\left(\frac12 +\frac{\delta}{4} +\mathcal{O}(\delta^2)\right) \cdot
\left(\frac1b + \delta\frac{(a+1)(b-1)}{2b} + \mathcal{O}(\delta^2)\right)
= \frac1N + \delta\cdot \frac{(a+1)(b-1)+1}{8b} + \mathcal{O}(\delta^2).\\
&=\frac1N + \delta\cdot\frac{N-2}{16} +\mathcal{O}(\delta^2).
\end{align*}


Thus we have derived the following theorem.

\begin{theorem}\label{thm:positive-r1}
Fix $N=4k$. Then the metafan $\amp_N$ satisfies
\[
\slope(\amp_N) \ge \frac{N-2}{16}.
\]
% , \pepa{Have notation for slope.} as $\delta\to 0$, we have
% \[
% \fp(\amp_N,r=1+\delta) = \frac1N + \delta\cdot \frac{(a+1)(b-1)+1}{8b}.
% \]
\end{theorem}
% \begin{proof}
% \end{proof}

